LiteNeXt: A Novel Lightweight ConvMixer-based Model with Self-embedding Representation Parallel for Medical Image Segmentation

The emergence of deep learning techniques has advanced the image segmentation task, especially for medical images. Many neural network models have been introduced in the last decade bringing the automated segmentation accuracy close to manual segmentation. However, cutting-edge models like Transformer-based architectures rely on large scale annotated training data, and are generally designed with densely consecutive layers in the encoder, decoder, and skip connections resulting in large number of parameters. Additionally, for better performance, they often be pretrained on a larger data, thus requiring large memory size and increasing resource expenses. In this study, we propose a new lightweight but efficient model, namely LiteNeXt, based on convolutions and mixing modules with simplified decoder, for medical image segmentation. The model is trained from scratch with small amount of parameters (0.71M) and Giga Floating Point Operations Per Second (0.42). To handle boundary fuzzy as well as occlusion or clutter in objects especially in medical image regions, we propose the Marginal Weight Loss that can help effectively determine the marginal boundary between object and background. Additionally, the Self-embedding Representation Parallel technique is proposed as an innovative data augmentation strategy that utilizes the network architecture itself for self-learning augmentation, enhancing feature extraction robustness without external data. Experiments on public datasets including Data Science Bowls, GlaS, ISIC2018, PH2, Sunnybrook, and Lung X-ray data show promising results compared to other state-of-the-art CNN-based and Transformer-based architectures. Our code is released at: https://github.com/tranngocduvnvp/LiteNeXt.

==> references_ordered_converted.tex <==
\begin{thebibliography}{99}

\bibitem{unet} Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas, "U-Net: Convolutional Networks for Biomedical Image Segmentation," Medical Image Computing and Computer-Assisted Intervention, 2015, pp. 234--241.

\bibitem{pattern_fewshot} Haoliang Sun and Xiankai Lu and Haochen Wang and Yilong Yin and Xiantong Zhen and Cees G.M. Snoek and Ling Shao, "Attentional prototype inference for few-shot segmentation," Pattern Recognition, 2023, vol. 142, pp. 109726.

\bibitem{dong2017automatic} Dong, Hao and Yang, Guang and Liu, Fangde and Mo, Yuanhan and Guo, Yike, "Automatic Brain Tumor Detection and Segmentation Using U-Net Based Fully Convolutional Networks," Medical Image Understanding and Analysis, 2017, pp. 506--517.

\bibitem{deep_cascade_brain} Cui, Shaoguo and Mao, Lei and Jiang, Jingfeng and Liu, Chang and Xiong, Shuyu, "Automatic Semantic Segmentation of Brain Gliomas from MRI Images Using a Deep Cascaded Neural Network," Journal of Healthcare Engineering, 2018, vol. 2018, pp. 1-14.

\bibitem{isensee2018brain} Isensee, Fabian and Kickingereder, Philipp and Wick, Wolfgang and Bendszus, Martin and Maier-Hein, Klaus H., "Brain Tumor Segmentation and Radiomics Survival Prediction: Contribution to the BRATS 2017 Challenge," Brainlesion: Glioma, Multiple Sclerosis, Stroke and Traumatic Brain Injuries, 2018, pp. 287--297.

\bibitem{pattern_semi} Cheng Tang and Xinyi Zeng and Luping Zhou and Qizheng Zhou and Peng Wang and Xi Wu and Hongping Ren and Jiliu Zhou and Yan Wang, "Semi-supervised medical image segmentation via hard positives oriented contrastive learning," Pattern Recognition, 2024, vol. 146, pp. 110020.

\bibitem{blunet} Hongyang Zhang and Wenxue Zhang and Weihao Shen and Nana Li and Yunjie Chen and Shuo Li and Bo Chen and Shijie Guo and Yuanquan Wang, "Automatic segmentation of the cardiac MR images based on nested fully convolutional dense network with dilated convolution," Biomedical Signal Processing and Control, 2021, vol. 68, pp. 102684.

\bibitem{acdc} Bernard, Olivier and Lalande, Alain and Zotti, Clement and Cervenansky, Frederick and Yang, Xin and Heng, Pheng-Ann and Cetin, Irem and Lekadir, Karim and Camara, Oscar and Gonzalez Ballester, Miguel Angel and Sanroma, Gerard and Napel, Sandy and Petersen, Steffen and Tziritas, Georgios and Grinias, Elias and Khened, Mahendra and Kollerathu, Varghese Alex and Krishnamurthi, Ganapathy and Rohé, Marc-Michel and Pennec, Xavier and Sermesant, Maxime and Isensee, Fabian and Jäger, Paul and Maier-Hein, Klaus H. and Full, Peter M. and Wolf, Ivo and Engelhardt, Sandy and Baumgartner, Christian F. and Koch, Lisa M. and Wolterink, Jelmer M. and Išgum, Ivana and Jang, Yeonggul and Hong, Yoonmi and Patravali, Jay and Jain, Shubham and Humbert, Olivier and Jodoin, Pierre-Marc, "Deep Learning Techniques for Automatic MRI Cardiac Multi-Structures Segmentation and Diagnosis: Is the Problem Solved?," IEEE Transactions on Medical Imaging, 2018, vol. 37, no. 11, pp. 2514-2525.

\bibitem{nham22} Do-Hai-Ninh Nham and Minh-Nhat Trinh and Viet-Dung Nguyen and Van-Truong Pham and Thi-Thao Tran, "An EffcientNet-encoder U-Net Joint Residual Refinement Module with Tversky–Kahneman Baroni–Urbani–Buser loss for biomedical image Segmentation," Biomedical Signal Processing and Control, 2023, vol. 83, pp. 104631.

\bibitem{skin_diagnosis} Zhang, Ni and Cai, Yi-Xin and Wang, Yong-Yong and Tian, Yi-Tao and Wang, Xiao-Li and Badami, Benjamin, "Skin Cancer Diagnosis Based on Optimized Convolutional Neural Network," Artificial Intelligence in Medicine, 2019, vol. 102, pp. 101756.

\bibitem{nuclei_evaluation} Caicedo, Juan and Roth, Jonathan and Goodman, Allen and Becker, Tim and Karhohs, Kyle and Broisin, Matthieu and Molnar, Csaba and McQuin, Claire and Singh, Shantanu and Theis, Fabian and Carpenter, Anne, "Evaluation of Deep Learning Strategies for Nucleus Segmentation in Fluorescence Images," Cytometry Part A, 2019, vol. 95.

\bibitem{nucleus_exemplars} Feng, Linqing and Song, Jun Ho and Kim, Jiwon and Jeong, Soomin and Park, Jin Sung and Kim, Jinhyun, "Robust Nucleus Detection With Partially Labeled Exemplars," IEEE Access, 2019, vol. 7, pp. 162169-162178.

\bibitem{earnet} Pham, Van-Truong and Tran, Thi-Thao and Wang, Pa-Chun and Chen, Po-Yu and Lo, Men-Tzung, "EAR-UNet: A Deep Learning-based Approach for Segmentation of Tympanic Membranes from Otoscopic Images," Artificial Intelligence in Medicine, 2021, vol. 115, pp. 102065.

\bibitem{attentionunet} Ozan Oktay and Jo Schlemper and Loic Le Folgoc and Matthew Lee and Mattias Heinrich and Kazunari Misawa and Kensaku Mori and Steven McDonagh and Nils Y Hammerla and Bernhard Kainz and Ben Glocker and Daniel Rueckert, "Attention U-Net: Learning Where to Look for the Pancreas," Unknown Journal/Conference, 2018.

\bibitem{valanarasu2021medical} Valanarasu, Jeya Maria Jose and Oza, Poojan and Hacihaliloglu, Ilker and Patel, Vishal M, "Medical transformer: Gated axial-attention for medical image segmentation," Medical Image Computing and Computer Assisted Intervention--MICCAI 2021: 24th International Conference, Strasbourg, France, September 27--October 1, 2021, Proceedings, Part I 24, 2021, pp. 36--46.

\bibitem{valanarasu2022unext} Valanarasu, Jeya Maria Jose and Patel, Vishal M, "Unext: Mlp-based rapid medical image segmentation network," International Conference on Medical Image Computing and Computer-Assisted Intervention, 2022, pp. 23--33.

\bibitem{ronneberger2015u} Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas, "U-net: Convolutional networks for biomedical image segmentation," Medical Image Computing and Computer-Assisted Intervention--MICCAI 2015: 18th International Conference, Munich, Germany, October 5-9, 2015, Proceedings, Part III 18, 2015, pp. 234--241.

\bibitem{dinh20231m} Dinh, Binh-Duong and Nguyen, Thanh-Thu and Tran, Thi-Thao and Pham, Van-Truong, "1M parameters are enough? A lightweight CNN-based model for medical image segmentation," 2023 Asia Pacific Signal and Information Processing Association Annual Summit and Conference (APSIPA ASC), 2023, pp. 1279--1284.

\bibitem{xie2021segformer} Xie, Enze and Wang, Wenhai and Yu, Zhiding and Anandkumar, Anima and Alvarez, Jose M and Luo, Ping, "SegFormer: Simple and efficient design for semantic segmentation with transformers," Advances in Neural Information Processing Systems, 2021, vol. 34, pp. 12077--12090.

\bibitem{transunet} Jieneng Chen and Yongyi Lu and Qihang Yu and Xiangde Luo and Ehsan Adeli and Yan Wang and Le Lu and Alan L. Yuille and Yuyin Zhou, "TransUNet: Transformers Make Strong Encoders for Medical Image Segmentation," Unknown Journal/Conference, 2021.

\bibitem{swinunet} Hu Cao and Yueyue Wang and Joy Chen and Dongsheng Jiang and Xiaopeng Zhang and Qi Tian and Manning Wang, "Swin-Unet: Unet-like Pure Transformer for Medical Image Segmentation," Unknown Journal/Conference, 2021.

\bibitem{byol} Grill, Jean-Bastien and Strub, Florian and Altch{\'e}, Florent and Tallec, Corentin and Richemond, Pierre and Buchatskaya, Elena and Doersch, Carl and Avila Pires, Bernardo and Guo, Zhaohan and Gheshlaghi Azar, Mohammad and others, "Bootstrap your own latent-a new approach to self-supervised learning," Advances in neural information processing systems, 2020, vol. 33, pp. 21271--21284.

\bibitem{dosovitskiy2020image} Alexey Dosovitskiy and Lucas Beyer and Alexander Kolesnikov and Dirk Weissenborn and Xiaohua Zhai and Thomas Unterthiner and Mostafa Dehghani and Matthias Minderer and Georg Heigold and Sylvain Gelly and Jakob Uszkoreit and Neil Houlsby, "An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale," International Conference on Learning Representations, 2021.

\bibitem{pvit} Wang, Wenhai and Xie, Enze and Li, Xiang and Fan, Deng-Ping and Song, Kaitao and Liang, Ding and Lu, Tong and Luo, Ping and Shao, Ling, "Pyramid vision transformer: A versatile backbone for dense prediction without convolutions," Proceedings of the IEEE/CVF international conference on computer vision, 2021, pp. 568--578.

\bibitem{lai2022axial} Lai, Hong-Phuc and Tran, Thi-Thao and Pham, Van-Truong, "Axial attention mlp-mixer: A new architecture for image segmentation," 2022 IEEE Ninth International Conference on Communications and Electronics (ICCE), 2022, pp. 381--386.

\bibitem{mlpmixer} Tolstikhin, Ilya O and Houlsby, Neil and Kolesnikov, Alexander and Beyer, Lucas and Zhai, Xiaohua and Unterthiner, Thomas and Yung, Jessica and Steiner, Andreas and Keysers, Daniel and Uszkoreit, Jakob and others, "Mlp-mixer: An all-mlp architecture for vision," Advances in neural information processing systems, 2021, vol. 34, pp. 24261--24272.

\bibitem{convmixer} Trockman, Asher and Kolter, J Zico, "Patches are all you need?," arXiv preprint arXiv:2201.09792, 2022.

\bibitem{yu2022metaformer} Yu, Weihao and Luo, Mi and Zhou, Pan and Si, Chenyang and Zhou, Yichen and Wang, Xinchao and Feng, Jiashi and Yan, Shuicheng, "Metaformer is actually what you need for vision," Proceedings of the IEEE/CVF conference on computer vision and pattern recognition, 2022, pp. 10819--10829.

\bibitem{liu2022convnet} Liu, Zhuang and Mao, Hanzi and Wu, Chao-Yuan and Feichtenhofer, Christoph and Darrell, Trevor and Xie, Saining, "A convnet for the 2020s," Proceedings of the IEEE/CVF conference on computer vision and pattern recognition, 2022, pp. 11976--11986.

\bibitem{unet++} Zhou, Zongwei and Rahman Siddiquee, Md Mahfuzur and Tajbakhsh, Nima and Liang, Jianming, "Unet++: A nested u-net architecture for medical image segmentation," Deep Learning in Medical Image Analysis and Multimodal Learning for Clinical Decision Support: 4th International Workshop, DLMIA 2018, and 8th International Workshop, ML-CDS 2018, Held in Conjunction with MICCAI 2018, Granada, Spain, September 20, 2018, Proceedings 4, 2018, pp. 3--11.

\bibitem{Unetv3} Huang, Huimin and Lin, Lanfen and Tong, Ruofeng and Hu, Hongjie and Zhang, Qiaowei and Iwamoto, Yutaro and Han, Xianhua and Chen, Yen-Wei and Wu, Jian, "Unet 3+: A full-scale connected unet for medical image segmentation," ICASSP 2020-2020 IEEE international conference on acoustics, speech and signal processing (ICASSP), 2020, pp. 1055--1059.

\bibitem{wang2022uctransnet} Wang, Haonan and Cao, Peng and Wang, Jiaqi and Zaiane, Osmar R, "Uctransnet: rethinking the skip connections in u-net from a channel-wise perspective with transformer," Proceedings of the AAAI conference on artificial intelligence, 2022, vol. 36, no. 3, pp. 2441--2449.

\bibitem{tran2023multi} Tran, Ngoc-Du and Nguyen, Dinh-Quoc-Dai and Nguyen, Ngoc-Linh-Chi and Pham, Van-Truong and Tran, Thi-Thao, "A Multi Context Decoder-based Network with Applications for Polyp Segmentation in Colonoscopy Images," Conference on Information Technology and its Applications, 2023, pp. 157--168.

\bibitem{vaswani2017attention} Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia, "Attention is all you need," Advances in neural information processing systems, 2017, vol. 30.

\bibitem{yi2004automated} Yi-de, Ma and Qing, Liu and Zhi-Bai, Qian, "Automated image segmentation using improved PCNN model based on cross-entropy," Proceedings of 2004 International Symposium on Intelligent Multimedia, Video and Speech Processing, 2004., 2004, pp. 743--746.

\bibitem{WBCE} Pihur, Vasyl and Datta, Susmita and Datta, Somnath, "Weighted rank aggregation of cluster validation measures: a Monte Carlo cross-entropy approach," Bioinformatics, 2007, vol. 23, no. 13, pp. 1607--1615.

\bibitem{BBCE} Xie, Saining and Tu, Zhuowen, "Holistically-nested edge detection," Proceedings of the IEEE international conference on computer vision, 2015, pp. 1395--1403.

\bibitem{focalloss} Lin, Tsung-Yi and Goyal, Priya and Girshick, Ross and He, Kaiming and Doll{\'a}r, Piotr, "Focal loss for dense object detection," Proceedings of the IEEE international conference on computer vision, 2017, pp. 2980--2988.

\bibitem{chen2020simple} Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey, "A simple framework for contrastive learning of visual representations," International conference on machine learning, 2020, pp. 1597--1607.

\bibitem{ema} Hunter, J Stuart, "The exponentially weighted moving average," Journal of quality technology, 1986, vol. 18, no. 4, pp. 203--210.

\bibitem{rashno2017fully} Rashno, Abdolreza and Koozekanani, Dara D and Drayna, Paul M and Nazari, Behzad and Sadri, Saeed and Rabbani, Hossein and Parhi, Keshab K, "Fully automated segmentation of fluid/cyst regions in optical coherence tomography images with diabetic macular edema using neutrosophic sets and graph algorithms," IEEE Transactions on Biomedical Engineering, 2017, vol. 65, no. 5, pp. 989--1001.

\bibitem{codella2019skin} Codella, Noel and Rotemberg, Veronica and Tschandl, Philipp and Celebi, M Emre and Dusza, Stephen and Gutman, David and Helba, Brian and Kalloo, Aadi and Liopyris, Konstantinos and Marchetti, Michael and others, "Skin lesion analysis toward melanoma detection 2018: A challenge hosted by the international skin imaging collaboration (isic)," arXiv preprint arXiv:1902.03368, 2019.

\bibitem{gladseg} Sirinukunwattana, Korsuk and Pluim, Josien PW and Chen, Hao and Qi, Xiaojuan and Heng, Pheng-Ann and Guo, Yun Bo and Wang, Li Yang and Matuszewski, Bogdan J and Bruni, Elia and Sanchez, Urko and others, "Gland segmentation in colon histology images: The glas challenge contest," Medical image analysis, 2017, vol. 35, pp. 489--502.

\bibitem{mendoncca2013ph} Mendon{\c{c}}a, Teresa and Ferreira, Pedro M and Marques, Jorge S and Marcal, Andr{\'e} RS and Rozeira, Jorge, "PH 2-A dermoscopic image database for research and benchmarking," 2013 35th annual international conference of the IEEE engineering in medicine and biology society (EMBC), 2013, pp. 5437--5440.

\bibitem{radau2009evaluation} Radau, Perry and Lu, Yingli and Connelly, Kim and Paul, Gideon and Dick, Alexander J and Wright, Graham A, "Evaluation framework for algorithms segmenting short axis cardiac MRI.," The MIDAS Journal, 2009.

\bibitem{jaeger2013automatic} Jaeger, Stefan and Karargyris, Alexandros and Candemir, Sema and Folio, Les and Siegelman, Jenifer and Callaghan, Fiona and Xue, Zhiyun and Palaniappan, Kannappan and Singh, Rahul K and Antani, Sameer and others, "Automatic tuberculosis screening using chest radiographs," IEEE transactions on medical imaging, 2013, vol. 33, no. 2, pp. 233--245.

\bibitem{candemir2013lung} Candemir, Sema and Jaeger, Stefan and Palaniappan, Kannappan and Musco, Jonathan P and Singh, Rahul K and Xue, Zhiyun and Karargyris, Alexandros and Antani, Sameer and Thoma, George and McDonald, Clement J, "Lung segmentation in chest radiographs using anatomical atlases with nonrigid registration," IEEE transactions on medical imaging, 2013, vol. 33, no. 2, pp. 577--590.

\bibitem{rahman2020reliable} Rahman, Tawsifur and Khandakar, Amith and Kadir, Muhammad Abdul and Islam, Khandaker Rejaul and Islam, Khandakar F and Mazhar, Rashid and Hamid, Tahir and Islam, Mohammad Tariqul and Kashem, Saad and Mahbub, Zaid Bin and others, "Reliable tuberculosis detection using chest X-ray with deep learning, segmentation and visualization," Ieee Access, 2020, vol. 8, pp. 191586--191601.

\bibitem{jaeger2014two} Jaeger, Stefan and Candemir, Sema and Antani, Sameer and W{\'a}ng, Y{\`\i}-Xi{\'a}ng J and Lu, Pu-Xuan and Thoma, George, "Two public chest X-ray datasets for computer-aided screening of pulmonary diseases," Quantitative imaging in medicine and surgery, 2014, vol. 4, no. 6, pp. 475.

\bibitem{vinta2024segmentation} Vinta, Surendra Reddy and Lakshmi, B and Safali, M Aruna and Kumar, G Sai Chaitanya, "Segmentation and Classification of Interstitial Lung Diseases Based on Hybrid Deep Learning Network Model," IEEE Access, 2024.

\bibitem{dozat2016incorporating} Dozat, Timothy, "Incorporating nesterov momentum into adam," Unknown Journal/Conference, 2016.

\bibitem{hastie2020ridge} Hastie, Trevor, "Ridge regularization: An essential concept in data science," Technometrics, 2020, vol. 62, no. 4, pp. 426--433.

\bibitem{gaogpu2000} Gao, Yanjie and Liu, Yu and Zhang, Hongyu and Li, Zhengxian and Zhu, Yonghao and Lin, Haoxiang and Yang, Mao, "Estimating GPU memory consumption of deep learning models," Proceedings of the 28th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering, 2020, pp. 1342–1352, \href{https://doi.org/10.1145/3368089.3417050}{DOI}.

\bibitem{zhangnn2021} Zhang, Li Lyna and Han, Shihao and Wei, Jianyu and Zheng, Ningxin and Cao, Ting and Yang, Yuqing and Liu, Yunxin, "nn-Meter: towards accurate latency prediction of deep-learning model inference on diverse edge devices," Proceedings of the 19th Annual International Conference on Mobile Systems, Applications, and Services, 2021, pp. 81–93.

\bibitem{attentionunet} Ozan Oktay and Jo Schlemper and Loic Le Folgoc and Matthew Lee and Mattias Heinrich and Kazunari Misawa and Kensaku Mori and Steven McDonagh and Nils Y Hammerla and Bernhard Kainz and Ben Glocker and Daniel Rueckert, "Attention U-Net: Learning Where to Look for the Pancreas," Unknown Journal/Conference, 2018.

\bibitem{fcn} Phi Vu Tran, "A Fully Convolutional Neural Network for Cardiac Segmentation in Short-Axis MRI," Unknown Journal/Conference, 2017.

\bibitem{xu2023dcsau} Xu, Qing and Ma, Zhicheng and Na, HE and Duan, Wenting, "DCSAU-Net: A deeper and more compact split-attention U-Net for medical image segmentation," Computers in Biology and Medicine, 2023, vol. 154, pp. 106626.

\bibitem{resunet} Diakogiannis, Foivos I. and Waldner, François and Caccetta, Peter and Wu, Chen, "ResUNet-a: A deep learning framework for semantic segmentation of remotely sensed data," ISPRS Journal of Photogrammetry and Remote Sensing, 2020, vol. 162, pp. 94–114.

\bibitem{nnUnet} Isensee, Fabian and Jaeger, Paul F and Kohl, Simon AA and Petersen, Jens and Maier-Hein, Klaus H, "nnU-Net: a self-configuring method for deep learning-based biomedical image segmentation," Nature methods, 2021, vol. 18, no. 2, pp. 203--211.

\bibitem{unetv2} Yaopeng Peng and Milan Sonka and Danny Z. Chen, "U-Net v2: Rethinking the Skip Connections of U-Net for Medical Image Segmentation," Unknown Journal/Conference, 2024.

\bibitem{vmUnetv2} "Zhang, Mingya, ""VM-UNET-V2: Rethinking Vision Mamba UNet for Medical Image Segmentation"," "Bioinformatics Research and Applications", "2024", pp. "335--346".

\bibitem{Unetv3} Huang, Huimin and Lin, Lanfen and Tong, Ruofeng and Hu, Hongjie and Zhang, Qiaowei and Iwamoto, Yutaro and Han, Xianhua and Chen, Yen-Wei and Wu, Jian, "Unet 3+: A full-scale connected unet for medical image segmentation," ICASSP 2020-2020 IEEE international conference on acoustics, speech and signal processing (ICASSP), 2020, pp. 1055--1059.

\bibitem{msrfnet} Abhishek Srivastava and Debesh Jha and Sukalpa Chanda and Umapada Pal and Haavard D. Johansen and Dag Johansen and M. Riegler and Sharib Ali and Paal Halvorsen, "MSRF-Net: A Multi-Scale Residual Fusion Network for Biomedical Image Segmentation," IEEE Journal of Biomedical and Health Informatics, 2022, vol. 26, pp. 2252-2263.

\bibitem{doubleunet} D. Jha and M. A. Riegler and D. Johansen and P. Halvorsen and H. D. Johansen, "DoubleU-Net: A Deep Convolutional Neural Network for Medical Image Segmentation," 2020 IEEE 33rd International Symposium on Computer-Based Medical Systems (CBMS), 2020, pp. 558-564.

\bibitem{deeplabv3} Chen, Liang-Chieh and Papandreou, George and Schroff, Florian and Adam, Hartwig, "Rethinking atrous convolution for semantic image segmentation," arXiv preprint arXiv:1706.05587, 2017.

\bibitem{badrinarayanan2017segnet} Badrinarayanan, Vijay and Kendall, Alex and Cipolla, Roberto, "Segnet: A deep convolutional encoder-decoder architecture for image segmentation," IEEE transactions on pattern analysis and machine intelligence, 2017, vol. 39, no. 12, pp. 2481--2495.

\bibitem{hasan2020dsnet} Hasan, Md Kamrul and Dahal, Lavsen and Samarakoon, Prasad N and Tushar, Fakrul Islam and Mart{\'\i}, Robert, "DSNet: Automatic dermoscopic skin lesion segmentation," Computers in biology and medicine, 2020, vol. 120, pp. 103738.

\bibitem{goyal2019skin} Goyal, Manu and Oakley, Amanda and Bansal, Priyanka and Dancey, Darren and Yap, Moi Hoon, "Skin lesion segmentation in dermoscopic images with ensemble deep learning methods," IEEE Access, 2019, vol. 8, pp. 4171--4181.

\bibitem{ozturk2020skin} \"O}zt{\"u}rk, {\c{S}}aban and {\"O}zkaya, Umut, "Skin lesion segmentation with improved convolutional neural network," Journal of digital imaging, 2020, vol. 33, pp. 958--970.

\bibitem{unver2019skin} \"U}nver, Halil Murat and Ayan, Enes, "Skin lesion segmentation in dermoscopic images with combination of YOLO and grabcut algorithm," Diagnostics, 2019, vol. 9, no. 3, pp. 72.

\bibitem{BCE} Yi-de, Ma and Qing, Liu and Zhi-Bai, Qian, "Automated image segmentation using improved PCNN model based on cross-entropy," Proceedings of 2004 International Symposium on Intelligent Multimedia, Video and Speech Processing, 2004., 2004, pp. 743--746.

\end{thebibliography}
